EarthDial: Turning Multi-sensory Earth Observations to Interactive Dialogues

Automated analysis of vast Earth observation data via interactive Vision-Language Models (VLMs) can unlock new opportunities for environmental monitoring, disaster response, and {resource management}. Existing generic VLMs do not perform well on Remote Sensing data, while the recent Geo-spatial VLMs remain restricted to a fixed resolution and few sensor modalities. In this paper, we introduce EarthDial, a conversational assistant specifically designed for Earth Observation (EO) data, transforming complex, multi-sensory Earth observations into interactive, natural language dialogues. EarthDial supports multi-spectral, multi-temporal, and multi-resolution imagery, enabling a wide range of remote sensing tasks, including classification, detection, captioning, question answering, visual reasoning, and visual grounding. To achieve this, we introduce an extensive instruction tuning dataset comprising over 11.11M instruction pairs covering RGB, Synthetic Aperture Radar (SAR), and multispectral modalities such as Near-Infrared (NIR) and infrared. Furthermore, EarthDial handles bi-temporal and multi-temporal sequence analysis for applications like change detection. Our extensive experimental results on 44 downstream datasets demonstrate that EarthDial outperforms existing generic and domain-specific models, achieving better generalization across various EO tasks. Our source codes and pre-trained models are at https://github.com/hiyamdebary/EarthDial.

==> tables/MS_classification.tex <==

\begin{table}[t]
    \centering
    \caption{Performance evaluation of the proposed EarthDial across diverse modalities for multi-class classification and referred object detection tasks on SAR imagery. On BigEarthNet, EarthDial achieves a 1.75\% improvement in classification accuracy using a fusion strategy. For SAR imagery, EarthDial delivers higher mAP, even when detecting multiple objects, highlighting the advantages of leveraging multi-modal inputs for enhanced accuracy.}
    \vspace{-0.3cm}\setlength{\tabcolsep}{3pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccc}
    \toprule
        \multicolumn{2}{c}{BigEarthNet~\cite{sumbul2019bigearthnet}} & SoSAT-LCZ42~\cite{zhu2019so2sat}  & TreeSatAI~\cite{astruc2024omnisat} & \multicolumn{5}{c}{Ship Dataset (SAR Imagery)} \\
        RGB & MS & MS & RGBI & Small & Medium & Large & Single & Multiple \\
        \midrule
        68.19 & 69.94 & 59.59 & 56.93 & 27.10 & 45.12 & 66.6 & 44.10 & 27.17\\
        
    \bottomrule
\end{tabular}}
\label{tab:ms_classification}
\end{table}

==> tables/token_format_table.tex <==
\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l l}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Token format}                            & \textbf{Description}                           \\ \hline
{[}s2\_rgb\_10{]}                                & Sentinel-2 RGB, 10m resolution (16-bit)        \\
 {[}s2\_ms\_10{]}              & Sentinel-2 multispectral, 10m (16-bit)  \\
 {[}l8\_rgb\_30{]}                                & Landsat 8 RGB, 30m resolution (16-bit)         \\
 {[}l8\_ms\_30{]}                                 & Landsat 8 multispectral, 30m resolution (16-bit) \\
 {[}s1\_vh\_1{]}                                 & Sentinel-1 VH polarization, 1m resolution (16-bit), SAR \\
 {[}s1\_vh\_10{]}                                 & Sentinel-1 VH polarization, 10m resolution (16-bit), SAR \\
 {[}s1\_vh\_temp\_10{]}                                 & Temporal Sentinel-1 VH polarization, 10m resolution (16-bit), SAR \\
{[}hr\_rgb\_0.5{]}                               & NAIP RGB, 0.5m resolution (8-bit)              \\
 {[}hr\_rgb\_0.5{]}                               & RGB, 0.5m resolution              \\
 {[}hr\_rgbi\_0.5{]}                               & RGB, Near-Infrared 0.5m resolution              \\
{[}hr\_rgb\_temp\_0.5{]}                               & Temporal RGB, 0.5m resolution              \\
 {[}Inf\_thermal\_1{]}                                & Infrared thermal, 1m resolution          \\
{[}hyper\_rgb\_3{]}                                &  Hyperspectral (AVIRIS-NG), 3m resolution   (8-bit)         \\
\hline
\end{tabular}
}
\caption{Overview of datasets with respective token formats and descriptions. This table lists key satellite datasets along with their token formats, resolutions, bit depths, and specific applications such as LULC and UHI detection.}
\label{tab:datasets}
\end{table}

==> tikz/primary_figure.tex <==
\begin{tikzpicture}

% \node[anchor=center] (earth) at (0, 0) {\includegraphics[width=4cm]{tikz/earth.png}}; 

\node[anchor=center] (earth) at (0, 0) {\includegraphics[width=1.55cm]{tikz/logo.jpeg}};  

\def\outerRadius{6}
\def\innerRadius{3.5} 
\def\globeRadius{1} 
\def\textRadiusTop{3.85} 
\def\textRadiusInnerBottom{2.75}
\def\spaceBetween{2} 
\def\numTopSegments{5}
\def\numBottomSegments{5}

\def\topLabels{{SAR, RGB, Multi-Spectral, Multi-Temporal, High resolution}}
\def\bottomLabels{{Classification, Captioning, VQA, Grounding, Detection}}
\def\innerBottomLabels{{Subtask 1, Subtask 2, Subtask 3, Subtask 4, Subtask 5, Subtask 6, Subtask 7, Subtask 8, Subtask 9, Subtask 10}} 

% Define dynamically calculated text width values
\pgfmathsetmacro{\topTextWidth}{(\outerRadius - \globeRadius)}
\pgfmathsetmacro{\bottomTextWidth}{(\outerRadius - \innerRadius) * 0.4}
% \pgfmathsetmacro{\innerTextWidth}{\innerRadiusExtended * 0.6}

\foreach \i [count=\j from 0] in {SAR \includegraphics[width=0.4cm]{tikz/satellite_1f6f0-fe0f.png}, RGB \includegraphics[width=0.4cm]{tikz/camera_1f4f7.png}, \includegraphics[width=0.4cm]{tikz/rainbow_1f308.png} Multi-Spectral, \includegraphics[width=0.4cm]{tikz/hourglass-not-done_23f3.png} Multi-Temporal, \includegraphics[width=0.4cm]{tikz/magnifying-glass-tilted-left_1f50d.png} High resolution} {
    \pgfmathsetmacro{\startAngle}{(\j * (180 / \numTopSegments)) - 90 + \spaceBetween/2}
    \pgfmathsetmacro{\endAngle}{((\j + 1) * (180 / \numTopSegments)) - 90 - \spaceBetween/2}
    \pgfmathsetmacro{\midAngle}{(\startAngle + \endAngle) / 2}
    \pgfmathsetmacro{\finalAngle}{\midAngle - 90}
    \ifdim \finalAngle pt > 90 pt \pgfmathsetmacro{\finalAngle}{\finalAngle - 180} \fi
    \ifdim \finalAngle pt < -90 pt \pgfmathsetmacro{\finalAngle}{\finalAngle + 180} \fi
    \draw[thick, fill=orange!20] 
        ({\startAngle + 90}:\globeRadius) arc[start angle={\startAngle + 90}, end angle={\endAngle + 90}, radius=\globeRadius]
        -- ({\endAngle + 90}:\outerRadius) arc[start angle={\endAngle + 90}, end angle={\startAngle + 90}, radius=\outerRadius]
        -- cycle;

    \node[text width=\topTextWidth cm, align=center, font=\normalsize, rotate=\finalAngle, anchor=center] at ({\midAngle + 90}:\globeRadius*0.5+\outerRadius*0.5) {\i};
}

\foreach \i [count=\j from 0] in {Classification, Captioning, VQA, Grounding, Detection} {
    \pgfmathsetmacro{\startAngle}{(\j * (180 / \numBottomSegments)) + 90 + \spaceBetween/2}
    \pgfmathsetmacro{\endAngle}{((\j + 1) * (180 / \numBottomSegments)) + 90 - \spaceBetween/2}
    \pgfmathsetmacro{\midAngle}{(\startAngle + \endAngle) / 2}
    
    % Rotate text perpendicular to the axis of each trapezoid
    \pgfmathsetmacro{\rotAngle}{\midAngle + 90}

    \draw[thick, fill=yellow!50] 
        ({\startAngle + 90}:\innerRadius) arc[start angle={\startAngle + 90}, end angle={\endAngle + 90}, radius=\innerRadius] 
        -- ({\endAngle + 90}:\outerRadius) arc[start angle={\endAngle + 90}, end angle={\startAngle + 90}, radius=\outerRadius]
        -- cycle;

    % Rotate text perpendicular to the trapezoid axis
    \node[text width=2.1cm, align=center, font=\normalsize, rotate=\rotAngle + 90, anchor=center] at ({\midAngle + 90}:\outerRadius*0.6 +\innerRadius*0.5) {\i};
}

% Define dynamically calculated midpoint radius for centering text
\def\innerRadiusExtended{4.9}
\pgfmathsetmacro{\midRadius}{(\globeRadius + \innerRadiusExtended) / 2}

\foreach \i [count=\j from 0] in {Local Climate Zones, Tree Species, Environment monitoring, Precision farming, Disaster management, Urban planning, Object localization, Infrastructure development, Methane plume, Vehicle/ship} {
    \pgfmathsetmacro{\segmentIndex}{int(\j / 2)}
    \pgfmathsetmacro{\isFirstInPair}{mod(\j, 2) == 0}
    \pgfmathsetmacro{\pairStartAngle}{(\segmentIndex * (180 / \numBottomSegments)) + 90 + \spaceBetween/2}
    \pgfmathsetmacro{\pairEndAngle}{((\segmentIndex + 1) * (180 / \numBottomSegments)) + 90 - \spaceBetween/2}
    
    \ifnum\isFirstInPair=1
        \pgfmathsetmacro{\startAngle}{\pairStartAngle}
        \pgfmathsetmacro{\endAngle}{(\pairStartAngle + \pairEndAngle) / 2}
    \else
        \pgfmathsetmacro{\startAngle}{(\pairStartAngle + \pairEndAngle) / 2}
        \pgfmathsetmacro{\endAngle}{\pairEndAngle}
    \fi
    
    \pgfmathsetmacro{\midAngle}{(\startAngle + \endAngle) / 2}
    \pgfmathsetmacro{\rotAngle}{\midAngle - 90}
    
    % Draw the trapezoid with the extended radius
    \draw[thick, fill=orange!30] 
        ({\startAngle + 90}:\globeRadius) arc[start angle={\startAngle + 90}, end angle={\endAngle + 90}, radius=\globeRadius]
        -- ({\endAngle + 90}:\innerRadiusExtended) arc[start angle={\endAngle + 90}, end angle={\startAngle + 90}, radius=\innerRadiusExtended]
        -- cycle;

    \ifnum\segmentIndex>1
        \pgfmathsetmacro{\rotAngle}{\rotAngle + 180}
    \fi
    
    % Place text at the dynamically calculated midpoint radius
    \node[text width=\innerRadiusExtended*0.9 cm, align=center, font=\normalsize, rotate=\rotAngle, anchor=center] at ({\midAngle + 90}:\midRadius) {\i};
}

\draw[dashed] (-0.5-\outerRadius, 0) -- (-\innerRadius, 0);
\draw[dashed] (\innerRadius, 0) -- (\outerRadius, 0);

\node[rotate=90, anchor=west] at (-\outerRadius-0.25, 0.25) {Data Modalities};
\node[rotate=90, anchor=east] at (-\outerRadius-0.25, -0.25) {Tasks/Applications};

\end{tikzpicture}
